An optimal open-loop strategy for handling a flexible beam with a robot manipulator

Fast and safe manipulation of flexible objects with a robot manipulator necessitates measures to cope with vibrations. Existing approaches either increase the task execution time or require complex models and/or additional instrumentation to measure vibrations. This paper develops a model-based method that overcomes these limitations. It relies on a simple pendulum-like model for modeling the beam, open-loop optimal control for suppressing vibrations, and does not require any exteroceptive sensors. We experimentally show that the proposed method drastically reduces residual vibrations -- at least 90% -- and outperforms the commonly used input shaping (IS) for the same execution time. Besides, our method can also execute the task faster than IS with a minor reduction in vibration suppression performance. The proposed method facilitates the development of new solutions to a wide range of tasks that involve dynamic manipulation of flexible objects.

==> input_shaping.tex <==
\subsection{Input shaping basics}
\textcolor{red}{\textit{First to be eliminated in case there is not enough space.}}

In this paper we compare our method to the input shaping -- the veteran of the vibration suppression field -- and briefly introduce it here. 
The main idea of input shaping: if a linear system has been excited by an impulse then it is possible to find a sequence of impulses with different magnitudes and application times that result in cancellation of vibrations caused by an initial impulse. The strength of the input shaper is that it can be applied to any reference command to prevent vibrations in the system caused by that input. 

In input shaping timing and amplitude of impulses are computed based on a dimensionless parameter called the percentage of residual vibrations that is derived from impulse response of a linear system to a series of impulses \cite{Singer1990ishaping}
\begin{align}
    V(\omega_n, \zeta)  =  \sqrt{C(\omega_n, \zeta)^2 + S(\omega_n, \zeta)^2} \nonumber
\end{align}
The simplest input shaper -- zero vibration (ZV) input shaper -- constrains $V(\cdot)$ to 0, sum of impulses to 1 yielding a shaper with two impulses at $t_1 = 0$ and $t_2 = 0.5T_d$ and amplitudes
\begin{align} \label{eq:zv_ishaper}
    A_1 = \frac{1}{1+K},\ A_2 = \frac{K}{1+K},\ K = \text{e}^{-\frac{\pi \zeta}{\sqrt{1 - \zeta^2}}} \nonumber
\end{align}
where $T_d$ is the period of damped vibrations. The ZV shaper is very sensitive to parameter mismatch, especially to errors in the natural frequency. There are other types of input shapers: robust input shapers that are robust against parameter mismatch and negative shapers that leverage negative amplitude impulses. However, the more robust is the input shaper the slower it is and negative shapers excite higher frequencies and yield high rate of change of the input.
